Leveraging Slither and Interval Analysis to build a Static Analysis Tool

Even though much progress has been made in identifying and mitigating smart contract vulnerabilities, we often hear about coding or design issues leading to great financial losses. This paper presents our progress toward finding defects that are sometimes not detected or completely detected by state-of-the-art analysis tools. Although it is still in its incipient phase, we developed a working solution built on top of Slither that uses interval analysis to evaluate the contract state during the execution of each instruction. To improve the accuracy of our results, we extend interval analysis by also considering the constraints imposed by specific instructions. We present the current solution architecture in detail and show how it could be extended to other static analysis techniques, including how it can be integrated with other third-party tools. Our current benchmarks contain examples of smart contracts that highlight the potential of this approach to detect certain code defects.

==> eptcsdata.tex <==
\providecommand{\firstpage}{150}
\providecommand{\publicationstatus}{M. Marin, L. Leu\c{s}tean (Eds.):\\ 
8th Symposium on Working Formal Methods (FROM 2024)\\
EPTCS 410, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.410.10}{10.4204/EPTCS.410.10}}
\pdfoutput=1

